Multi-Tier Non-Terrestrial Networking for Disaster Communications: A Layered Clustering Approach

It is crucial to deploy temporary non-terrestrial networks (NTN) in disaster situations where terrestrial networks are no longer operable. Deploying uncrewed aerial vehicle base stations (UAV-BSs) can provide a radio access network (RAN); however, the backhaul link may also be damaged and unserviceable in such disaster conditions. In this regard, high-altitude platform stations (HAPS) spark attention as they can be deployed as super macro base stations (SMBS) and data centers. Therefore, in this study, we investigate a three-layer heterogeneous network with different topologies to prolong the lifespan of the temporary network by using UAV-BSs for RAN services and HAPS-SMBS as a backhaul. Furthermore, a two-layer clustering algorithm is proposed to handle the UAV-BS ad-hoc networking effectively.

==> bin.tex <==
% Since this is a scenario that requires emergency intervention, the energy consumption of UAVs was taken into account.

% The contributions of this study are summarized as follows:
% \begin{itemize}
%     \item UAVs are positioned to provide communication in a disaster scenario, and HAPS-SMBS has been investigated to provide backhaul link to UAVs.
%     \item A two-layer clustering is proposed both in the UEs layer and in the UAV layer.
%     \item To compare the results three scenarios and different cluster situations are examined. 
% \end{itemize}

% The rest of the paper is structured as the system model is presented in Section II, while the proposed methodology is introduced in Section III. Then, Section IV shows performance evaluation and lastly Section V concludes the paper. 

% In this section the network model of the study and energy consumption model is introduced.

%where $\overline{d}$ is the mean distance between UAVs and UEs and $\lambda_t$ is total load. $d_{x,k}$ and $d_{y,k}$ are distance between each NH-UAV and H-UAV and $d_{y,k}$ distance between UAV and HAPS, respectively.

%Note that, the aim of this study is to ensure that all UAVs provide service for a longer time since there is an emergency situation. Therefore, the energy consumption of NH-UAVs is calculated by subtracting the consumption of the H-UAV from the calculation. Thus the new equation becomes as follows:
%\begin{equation}
%    E_\text{p} = \sum_{k=1}^{N-1} (\lambda_k \overline{d_k}+\lambda_k d_{x,k}). 
%\end{equation}

%\begin{equation}
 %   E_\text{p} = \sum_{k=1}^N (\lambda_k \overline{d_k}+\lambda_k d_{x,k}+\lambda_t d_{y})  
%\end{equation}

%The simulation parameters are given in Table \ref{table:simparameter}
%\begin{table}[ht]
%\centering
%\caption{Simulation Parameters} \label{table:simparameter}
%%\begin{adjustbox}{width=\columnwidth,center}
%\begin{tabular}{ll}
%\textbf{Parameters} & \textbf{Values} \\ \hline
%Environment area    & 3000 m $\times$ 3000 m     \\
%HAPS altitude & 20 km \\
%UAV altitude  &  200 m  \\
%Number of UAV    & 12        \\
%Hotspot number & 10 \\
%\bottomrule
%\end{tabular}
%%\end{adjustbox}
%\end{table}
